ALPS: An Auto-Labeling and Pre-training Scheme for Remote Sensing Segmentation With Segment Anything Model

In the fast-growing field of Remote Sensing (RS) image analysis, the gap between massive unlabeled datasets and the ability to fully utilize these datasets for advanced RS analytics presents a significant challenge. To fill the gap, our work introduces an innovative auto-labeling framework named ALPS (Automatic Labeling for Pre-training in Segmentation), leveraging the Segment Anything Model (SAM) to predict precise pseudo-labels for RS images without necessitating prior annotations or additional prompts. The proposed pipeline significantly reduces the labor and resource demands traditionally associated with annotating RS datasets. By constructing two comprehensive pseudo-labeled RS datasets via ALPS for pre-training purposes, our approach enhances the performance of downstream tasks across various benchmarks, including iSAID and ISPRS Potsdam. Experiments demonstrate the effectiveness of our framework, showcasing its ability to generalize well across multiple tasks even under the scarcity of extensively annotated datasets, offering a scalable solution to automatic segmentation and annotation challenges in the field. In addition, the proposed a pipeline is flexible and can be applied to medical image segmentation, remarkably boosting the performance. Note that ALPS utilizes pre-trained SAM to semi-automatically annotate RS images without additional manual annotations. Though every component in the pipeline has bee well explored, integrating clustering algorithms with SAM and novel pseudo-label alignment significantly enhances RS segmentation, as an off-the-shelf tool for pre-training data preparation. Our source code is available at: https://github.com/StriveZs/ALPS.

==> table/sota_ablation_1.tex <==
\begin{table}[!t]
    \centering
    \scriptsize
    \begin{subtable}[t]{1 \linewidth}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|ccc|cccccccccccccccc|cc}  
        \toprule[1.2pt]
        Methods & Type & Pre-trained & Step & BG & SH & ST & BD & TC & BC & GTF & BR & LV & SV & HC & SP & RA & SBF & PL & HA & mIoU & mAcc \\
        \hline
        % \multirow{4}{*}{UperNet} 
        %     % & Baseline & - & 80k & 98.67 & 68.80 & 71.29 & 71.98 & 86.67 & 52.68 & 57.35 & 39.94 & 63.29 & 48.30 & 0.00 & 48.09 & 47.35 & 72.38 & 82.74 & 58.20 & 64.52 & 73.70 \\
        %     & Backbone & SAMRS* & 80k & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        %     & Backbone & SAMRS-PL & 80k & 98.42 & 58.44 & 63.38 & 67.39 & 84.42 & 42.98 & 45.68 & 29.86 & 56.85 & 33.61 & 0.00 & 45.76 & 40.94 & 65.49 & 78.43 & 50.37 & 57.47 & 64.68 \\
        %     \cline{2-22}
        %     & Overall & SAMRS* & 80k & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        %     & Overall & SAMRS-PL & 80k & 98.65 & 67.83 & 71.23 & 69.63 & 87.13 & 52.65 & 57.32 & 40.01 & 63.20 & 45.76 & 0.00 & 52.58 & 49.87 & 73.77 & 82.38 & 57.80 & 64.65 & 74.17 \\
        % \hline
        \multirow{4}{*}{Segformer} 
            & Backbone & SAMRS* & 160k & 98.73 & 70.31 & 73.40 & 79.52 & 88.01 & 63.13 & 63.73 & 47.40 & 63.47 & 46.03 & 0.00 & 47.82 & 65.59 & 76.93 & 83.53 & 59.40 & 64.19 & 75.04 \\
            & Backbone & SAMRS-PL & 160k & 98.76 & 72.67 & 72.81 & 80.57 & 88.14 & 63.45 & 65.50 & 41.55 & 63.68 & 46.55 & 0.00 & 48.53 & 72.16 & 78.78 & 83.70 & 58.33 & \textbf{64.70} & \textbf{75.97} \\
            \cline{2-22}
            & Overall & SAMRS* & 160k & 98.73 & 70.79 & 72.95 & 79.91 & 88.00 & 64.28 & 66.32 & 48.11 & 63.83 & 46.94 & 0.00 & 50.10 & 66.12 & 77.93 & 83.62 & 59.07 & 64.80 & 75.75 \\
            & Overall & SAMRS-PL & 160k & 98.76 & 72.32 & 73.57 & 80.03 & 89.05 & 64.76 & 65.6 & 46.68 & 63.05 & 46.75 & 0.00 & 46.98 & 75.53 & 78.91 & 83.67 & 59.84 & \textbf{65.35} & \textbf{76.53} \\    
            \bottomrule
         \end{tabular}
    }
    \caption{}
    \label{tab:Table.6}
    \vspace{-3mm}
    \end{subtable}
    \begin{subtable}[t]{1 \linewidth}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|ccc|cccccccccccccccc|cc} 
        \toprule[1.2pt]
        Methods & Type & Pre-trained & Step & BG & SH & ST & BD & TC & BC & GTF & BR & LV & SV & HC & SP & RA & SBF & PL & HA & mIoU & mAcc \\
        \hline
        % \multirow{4}{*}{UperNet} 
        %     & Backbone & Binary Mask & 80k & 96.98 & 25.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 19.82 & 0.12 & 0.00 & 0.00 & 0.00 & 0.00 & 0.23 & 17.81 & 10.03 & 11.97 \\
        %     & Backbone & iSAID-PL & 80k & 98.39 & 59.85 & 62.92 & 61.74 & 83.12 & 42.24 & 52.28 & 29.92 & 56.92 & 45.22 & 0.00 & 48.31 & 46.28 & 61.27 & 76.66 & 53.96 & 58.61 & 65.16 \\
        %     & Backbone & SAMRS-PL & 80k & 98.42 & 58.44 & 63.38 & 67.39 & 84.42 & 42.98 & 45.68 & 29.86 & 56.85 & 33.61 & 0.00 & 45.76 & 40.94 & 65.49 & 78.43 & 50.37 & 57.47 & 64.68 \\
        %     & Backbone & Mixed-PL  & 80k & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        % \hline
        \multirow{4}{*}{Segformer} 
            & Backbone & Binary Mask & 160k & 97.10 & 30.30 & 0.88 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 21.98 & 3.21 & 0.00 & 0.00 & 0.00 & 0.00 & 2.79 & 19.88 & 11.01 & 13.55 \\
            & Backbone & iSAID-PL & 160k & 98.73 & 70.18 & 73.17 & 77.31 & 88.04 & 61.73 & 64.38 & 46.31 & 63.12 & 46.88 & 0.00 & 50.12 & 70.33 & 78.48 & 83.27 & 56.81 & 64.30 & 75.34 \\
            & Backbone & SAMRS-PL & 160k & 98.76 & 72.67 & 72.81 & 80.57 & 88.14 & 63.45 & 65.50 & 41.55 & 63.68 & 46.55 & 0.00 & 48.53 & 72.16 & 78.78 & 83.70 & 58.33 & 64.70 & 75.97 \\
            & Backbone & Mixed-PL  & 160k & 98.74 & 71.35 & 72.21 & 81.78 & 88.41 & 60.48 & 66.30 & 47.64 & 62.95 & 46.19 & 0.00 & 49.53 & 72.60 & 77.71 & 83.22 & 59.53 & \textbf{64.91} & \textbf{76.04} \\
            \bottomrule
         \end{tabular}
    }
    \caption{}
    \label{tab:Table.4}
    \end{subtable}
    \vspace{-3mm}
    \caption{(a)~Quantitative results of different pre-training datasets constructed by different unsupervised manners. SAMRS* represent the data generated by Oriented RepPoints \& SAMRS framework. (b)~Quantitative results of different pre-trained schemes on the iSAID dataset.}\vspace{-5mm}
\end{table}
